Identification Capacity of the Discrete-Time Poisson Channel

Numerous applications in the field of molecular communications (MC) such as healthcare systems are often event-driven. The conventional Shannon capacity may not be the appropriate metric for assessing performance in such cases. We propose the identification (ID) capacity as an alternative metric. Particularly, we consider randomized identification (RI) over the discrete-time Poisson channel (DTPC), which is typically used as a model for MC systems that utilize molecule-counting receivers. In the ID paradigm, the receiver's focus is not on decoding the message sent. However, he wants to determine whether a message of particular significance to him has been sent or not. In contrast to Shannon transmission codes, the size of ID codes for a Discrete Memoryless Channel (DMC) grows doubly exponentially fast with the blocklength, if randomized encoding is used. In this paper, we derive the capacity formula for RI over the DTPC subject to some peak and average power constraints. Furthermore, we analyze the case of state-dependent DTPC.

==> figures/Gaussian_MIMO.tex <==
\tikzstyle{farbverlauf} = [ top color=white, bottom color=white!80!gray]
\tikzstyle{vectorarrow} = [thick, decoration={markings,mark=at position
   1 with {\arrow[semithick]{open triangle 60}}},
   double distance=1.4pt, shorten >= 5.5pt,
   preaction = {decorate},
   postaction = {draw,line width=1.4pt, white,shorten >= 4.5pt}]
\tikzstyle{block} = [draw,top color=white, bottom color=white!80!gray, rectangle, rounded corners,
minimum height=2em, minimum width=2.5em]
\tikzstyle{input} = [coordinate]
\tikzstyle{sum} = [draw, circle,inner sep=0pt, minimum size=2mm,  thick]
\tikzstyle{arrow}=[draw,->] %{Latex[length=3mm]},
\scalebox{.87}{
\begin{tikzpicture}[auto, node distance=2cm,>=latex']
\node[] (M) {$M$};
\node[block,right=.4cm of M] (enc) {Encoder};
\node[block,right=.7cm of enc] (channel) {\large$\mathbf{H}$};
\node[sum, right=.7cm of channel] (sum) {$+$};
\node[block, right=.7cm of sum] (dec) {Decoder};
\node[right=.4cm of dec] (Mhat) {\begin{tabular}{c} Is $M^\prime$ sent? \\ Yes or No? \end{tabular}};
\node[above=.5cm of sum] (noise) {$\boldsymbol{\xi}$};
\draw[->] (M)--(enc);
\draw[vectorarrow] (enc) --node[above]{$\boldsymbol{x}$} (channel);
\draw[vectorarrow] (channel) -- (sum);
\draw[vectorarrow] (noise) -- (sum);
\draw[vectorarrow] (sum) -- node[above]{$\boldsymbol{y}$} (dec);
\draw[->] (dec) -- (Mhat) {};
\end{tikzpicture}}
